Exploring Ordinality in Text Classification: A Comparative Study of Explicit and Implicit Techniques

Ordinal Classification (OC) is a widely encountered challenge in Natural Language Processing (NLP), with applications in various domains such as sentiment analysis, rating prediction, and more. Previous approaches to tackle OC have primarily focused on modifying existing or creating novel loss functions that \textbf{explicitly} account for the ordinal nature of labels. However, with the advent of Pretrained Language Models (PLMs), it became possible to tackle ordinality through the \textbf{implicit} semantics of the labels as well. This paper provides a comprehensive theoretical and empirical examination of both these approaches. Furthermore, we also offer strategic recommendations regarding the most effective approach to adopt based on specific settings.

==> backup_table.tex <==
\begin{table*}[t]


\scriptsize
\addtolength{\tabcolsep}{-3pt}    
\begin{tabular}{clx{0.65cm}x{0.65cm}x{0.65cm}x{0.65cm}@{\hskip 0.2in}x{0.65cm}x{0.65cm}x{0.65cm}x{0.65cm}@{\hskip 0.2in}x{0.65cm}x{0.65cm}x{0.65cm}x{0.65cm}@{\hskip 0.2in}x{0.65cm}x{0.65cm}x{0.65cm}x{0.65cm}}

 &     & \multicolumn{4}{c}{100 \%} & \multicolumn{4}{c}{50 \%} &   \multicolumn{4}{c}{25 \%} &   \multicolumn{4}{c}{10 \%} \\
  &     & CE   & MLL   & ENT & GPT  &   CE   & MLL   & ENT   & GPT   &   CE   & MLL   & ENT  & GPT  &   CE   & MLL   & ENT   & GPT  \\ \hline
 \multirow{4}{*}{\rotatebox{90}{SNLI}} & F1 & 0.890  (0.02) &  \cellcolor{green!=45}0.891 (0.02) & 0.885 (0.30) & 0.776 (0.00) &   0.873 (0.00) &  0.882 (0.09) & \cellcolor{green!=45}0.885 (0.04) & 0.654 (0.00) &   0.861 (0.00)  & 0.865 (0.01) & \cellcolor{green!=45}0.869 (0.03) & 0.527 (0.01) &  0.836 (0.00) & \cellcolor{green!=45}0.848 (0.04) & 0.845 (0.01) & 0.389 (0.01) \\
 & MAE & 0.123 (0.01) & \cellcolor{green!=45}0.122 (0.02) & 0.128 (0.00) & 0.261 (0.00) &  0.146 (0.00) & 0.131 (0.11) & \cellcolor{green!=45}0.129 (0.00)  & 0.424 (0.00)  &      0.161 (0.00)    & 0.153 (0.01) & \cellcolor{green!=45}  0.150 (0.00)   &  0.599 (0.02)  &   0.191 (0.00) & \cellcolor{green!=45} 0.171 (0.05) & 0.181 (0.00)  & 0.811 (0.01)\\
 & MSE & 0.152 (0.04) & \cellcolor{green!=45}0.149 (0.04) & 0.157 (0.01) & 0.338 (0.00) &  0.188 (0.00) & \cellcolor{green!=45} 0.156 (0.05)      & 0.159 (0.00) &   0.596 (0.00)  &  0.206 (0.00)     & \cellcolor{green!=30}0.190 (0.00) &  \cellcolor{green!=30}0.190 (0.00)   & 0.878 (0.04)   &    0.249 (0.01)  & 0.210 (0.06)  & \cellcolor{green!=45}0.236 (0.00)  & 1.263 (0.04)\\
 & OK1 & 0.985 (0.01) & \cellcolor{green!=45}0.986 (0.01)  & 0.985 (0.02) & 0.961 (0.00)  &  0.979 (0.00) & \cellcolor{green!=45}0.987 (0.02)      &  0.980 (0.00)  & 0.913 (0.00)    &      0.977 (0.00)     &  \cellcolor{green!=45}0.981 (0.02)    & 0.980 (0.00)   & 0.860 (0.01)      &       0.971 (0.00) & \cellcolor{green!=45}0.980 (0.00) & 0.972 (0.00)  & 0.774 (0.01) \\
\hline
\multirow{4}{*}{\rotatebox{90}{YELP}} & F1 & 0.635 (0.02) & \cellcolor{green!=45}0.638 (0.02) & 0.635 (0.03)   & 0.601 (0.00)  &  0.618 (0.02)  &  \cellcolor{green!=45} 0.624 (0.02) & 0.620 (0.54)   & 0.536 (0.00) &       0.602 (0.02)    & \cellcolor{green!=45}0.607 (0.02) &  0.602 (0.00)      &  0.431 (0.00)   &   0.581 (0.02) & 0.585 (0.02) & \cellcolor{green!=45}0.590 (0.01)  & 0.376 (0.05)  \\
 & MAE & 0.413 (0.06) & \cellcolor{green!=45}0.407 (0.01) & 0.417 (0.05)  & 0.447 (0.01) & 0.438 (0.02)   & \cellcolor{green!=45} 0.426 (0.02) &   0.437 (0.00)    &  0.527 (0.00)    &    0.463 (0.03)     &  \cellcolor{green!=45} 0.453 (0.04)    & 0.466 (0.01)    &   0.644 (0.00)    &   0.500 (0.02) & 0.487 (0.05) & \cellcolor{green!=45}0.477 (0.01)  & 0.633 (0.07)  \\
 & MSE & 0.539 (0.03) & \cellcolor{green!=45}0.518 (0.01) & 0.561 (0.01)  & 0.595 (0.02)  &  0.592 (0.06)    & \cellcolor{green!=45} 0.555 (0.05) & 0.596 (0.02)      &  0.749 (0.00)    &    0.643 (0.02)  & \cellcolor{green!=45}0.602 (0.02)  &  0.663 (0.03)   &    0.999 (0.00)   & 0.731 (0.02) &  0.674 (0.03) & \cellcolor{green!=45}0.65 (0.02) & 0.834 (0.15) \\
 & OK1 & 0.963 (0.01) & \cellcolor{green!=45}0.965 (0.03) & 0.960 (0.01) & 0.955 (0.00)  & 0.957 (0.00)      &  \cellcolor{green!=45}0.960 (0.08)   & 0.956 (0.00)    & 0.928 (0.00)   &     0.951 (0.00)  & \cellcolor{green!=45}0.956 (0.01)  &  0.946 (0.00)  & 0.883 (0.00)  &      0.941 (0.00)  & 0.949 (0.00) & \cellcolor{green!=45}0.952 (0.00) & 0.929 (0.02)  \\
\hline
\multirow{4}{*}{\rotatebox{90}{SST5}} & F1  & 0.484 (0.01) & 0.491 (0.02) & \cellcolor{green!=45}0.508 (0.01)  & 0.487 (0.02)  &     0.442 (0.02)    &   0.468 (0.03)    &  0.445 (0.02)      &  \cellcolor{green!=45}0.476 (0.00) &         0.415 (0.03)    & \cellcolor{green!=45}0.440 (0.04) &  0.423 (0.03)     & 0.316 (0.01) &   0.417 (0.02)  & 0.428 (0.02) & \cellcolor{green!=45}0.430 (0.03)  & 0.274 (0.02)\\
 & MAE & 0.576 (0.02) & 0.574 (0.01)  & \cellcolor{green!=45}0.543 (0.01)  & 0.585 (0.01)  &   0.620 (0.01)    &   0.600 (0.02)     &  \cellcolor{green!=45}0.585 (0.01)   & 0.595 (0.00)   &          0.652 (0.04)     &   0.620 (0.04)    & \cellcolor{green!=45}0.619 (0.04)     &  0.966 (0.03)  &      0.697 (0.02) & 0.662 (0.01) & \cellcolor{green!=45}0.651 (0.10)  & 1.043 (0.02) \\
 & MSE & 0.760 (0.02) & 0.756 (0.02) & 0.683 (0.02)    & 0.802 (0.02) &     0.845 (0.04)   & 0.760 (0.04)      &  0.794 (0.04)   &  0.819 (0.01)   &           0.910 (0.10)    &   0.827 (0.01)    & 0.870 (0.12)  & 1.740 (0.10)   &     1.04 (0.06) & 0.905 (0.01) & 0.871 (0.25)  & 1.897 (0.19) \\
 & OK1 &   0.925 (0.01)   &    0.931 (0.02)   &  0.932 (0.01)   & 0.918 (0.00)  &    0.910 (0.08) &      0.929 (0.01)      &  0.927 (0.01)   & 0.912 (0.00) &       0.902 (0.01)    &    0.918 (0.02)   & 0.911 (0.02)  & 0.769 (0.01)         &     0.875 (0.01) & 0.898 (0.02) & 0.915 (0.05)  & 0.734 (0.01)  \\
\hline
\multirow{4}{*}{\rotatebox{90}{ \parbox{1.5cm}{Amazon \newline Reviews} }} & F1  & 0.586 (0.04) & \cellcolor{green!=45}0.589 (0.04) & 0.585 (0.03)   & 0.522 (0.00)   &   0.573 (0.00)  & 0.579 (0.01) &  0.586 (0.02) & 0.449 (0.01)     &       0.563 (0.00)      &   0.572 (0.02)  &  0.572 (0.01)  & 0.402 (0.00) &       0.534 (0.01)  & 0.553 (0.03)  & 0.544 (0.01)  & 0.389 (0.00)\\
 & MAE & 0.485 (0.06) & \cellcolor{green!=45}0.476 (0.06)  &  0.483 (0.01) &  0.573 (0.01) &    0.505 (0.00) &  0.497 (0.01) & 0.480 (0.00)  & 0.678 (0.00)  &        0.520 (0.00)    &   0.503 (0.07)    &  0.502 (0.02)  & 0.773 (0.00) &    0.56 (0.01) & 0.528 (0.05) & 0.541 (0.02)  & 0.813 (0.00) \\
 & MSE & 0.675 (0.01) & \cellcolor{green!=45}0.634 (0.01) & 0.664 (0.02)  & 0.848 (0.04)   &      0.707 (0.01) & 0.683 (0.03)    &   0.655 (0.01)  & 1.085 (0.01)   &         0.739 (0.02)      &   0.689 (0.02)    & 0.698 (0.05)  &  1.348 (0.01)  &     0.835 (0.04) & 0.708 (0.01) & 0.767 (0.06)  & 1.475 (0.01) \\
 & OK1 & 0.938 (0.03) & \cellcolor{green!=45}0.945 (0.03) & 0.939 (0.01) & 0.911 (0.00)   &      0.932 (0.00)  &  0.935 (0.00)    &  \cellcolor{green!=45} 0.942 (0.00)  & 0.864 (0.00)   &       0.929 (0.00)     &    \cellcolor{green!=45}0.938 (0.03)   & 0.935 (0.01)  &  0.825 (0.00)  &   0.913 (0.00) & \cellcolor{green!=45}0.934 (0.02) & 0.925 (0.01) & 0.807 (0.00) \\
\hline

\end{tabular}
\caption{\small We report F1, MAE, MSE, OB1 metrics for all 4 datasets in full-data and few-shot settings. We include cross-entropy (CE) baseline, best performing explicit loss (MLL), Entailment technique (ENT) and Generative technique (GPT).}
\label{tab:main_table_real}
\addtolength{\tabcolsep}{3pt}    
\end{table*}


==> mae_plots_uninformed_vs_informed.tex <==



\begin{figure}[H]
\centering
\begin{minipage}{.24\textwidth}
  \centering
  \includegraphics[width=\linewidth]{SNLI_MAE.pdf}
  \label{fig:test11}
\end{minipage}%


\begin{minipage}{.24\textwidth}
  \centering
  \includegraphics[width=\linewidth]{SST5_MAE.pdf}
  \label{fig:test21}
\end{minipage}%
\begin{minipage}{.24\textwidth}
  \centering
  \includegraphics[width=\linewidth]{amazon_review_MAE.pdf}
  \label{fig:test22}
\end{minipage}%
\caption{\small Effect of informative vs non-informative prompts on ordinal metric (MAE).}
\label{fig:mae_random}
\end{figure}


==> main_bert_tiny_table.tex <==
\begin{table}[!ht]
\tiny
    \centering
    \begin{tabular}{c|cccccc}
        \textbf{Dataset} & \textbf{Loss } & \textbf{LR} & \textbf{F1} & \textbf{MSE} & 
        \textbf{MAE} & \textbf{O1} \\ \hline 
        \textbf{Yelp} & CE & 0.0001 & 0.579 & 0.789 & 0.520 & 0.926 \\ 
        \textbf{} & MLL & 0.0001 & 0.594 & 0.665 & 0.481 & 0.932 \\ 
        \textbf{} & OLL & 0.000075 & 0.567 & 0.708 & 0.518 & 0.924 \\ 
        \textbf{} & SOFT & 0.00005 & 0.575 & 0.803 & 0.526 & 0.929 \\ 
        \textbf{} & EMD & 0.00005 & 0.574 & 0.783 & 0.524 & 0.930 \\ 
        \textbf{} & ~ & ~ & ~ & ~ & ~ & ~ \\ 
        \textbf{SST5} & CE & 0.000025 & 0.357 & 1.197 & 0.768 & 0.852 \\ 
        \textbf{} & MLL & 0.0001 & 0.378 & 1.125 & 0.742 & 0.863 \\ 
        \textbf{} & OLL & 0.000025 & 0.359 & 1.055 & 0.740 & 0.870 \\ 
        \textbf{} & SOFT & 0.0001 & 0.382 & 1.152 & 0.751 & 0.856 \\ 
        \textbf{} & EMD & 0.0001 & 0.354 & 1.125 & 0.744 & 0.857 \\ 
        \textbf{} & ~ & ~ & ~ & ~ & ~ & ~ \\ 
        \textbf{Amazon reviews} & CE & 0.0001 & 0.543 & 0.904 & 0.581 & 0.903 \\ 
        \textbf{} & MLL & 0.000075 & 0.544 & 0.819 & 0.568 & 0.915 \\ 
        \textbf{} & OLL & 0.0001 & 0.530 & 0.788 & 0.571 & 0.924 \\ 
        \textbf{} & SOFT & 0.000075 & 0.537 & 0.904 & 0.586 & 0.903 \\ 
        \textbf{} & EMD & 0.00005 & 0.534 & 0.885 & 0.584 & 0.904 \\ 
        \textbf{} & ~ & ~ & ~ & ~ & ~ & ~ \\ 
        \textbf{SNLI} & CE & 0.00005 & 0.821 & 0.264 & 0.208 & 0.972 \\ 
        \textbf{} & MLL & 0.000075 & 0.832 & 0.257 & 0.205 & 0.974 \\ 
        \textbf{} & OLL & 0.0001 & 0.803 & 0.250 & 0.217 & 0.980 \\ 
        \textbf{} & SOFT & 0.0001 & 0.824 & 0.257 & 0.203 & 0.972 \\ 
        \textbf{} & EMD & 0.0001 & 0.826 & 0.250 & 0.199 & 0.975 \\ 
    \end{tabular}
    \caption{Loss functions comparison on four datasets using TinyBERT architecture}
    \label{tab:mainpaper-losses-bert-tiny}
\end{table}


==> main_table.tex <==
\begin{table*}[]
\tiny
\begin{tabular}{cp{0.20cm}p{0.20cm}p{0.20cm}p{0.20cm}p{0.20cm}p{0.20cm}p{0.20cm}|p{0.005cm}|p{0.20cm}p{0.20cm}p{0.20cm}p{0.20cm}p{0.20cm}p{0.20cm}|p{0.05cm}|p{0.20cm}p{0.20cm}p{0.20cm}p{0.20cm}p{0.20cm}p{0.20cm}|p{0.05cm}|p{0.20cm}p{0.20cm}p{0.20cm}p{0.20cm}p{0.20cm}p{0.20cm}}
 &     & \multicolumn{6}{c}{100 \%} &  & \multicolumn{6}{c}{50 \%} &  & \multicolumn{6}{c}{25 \%} &  & \multicolumn{6}{c}{10 \%} \\
  &     & CE   & MLL   & B & B-U & GPT  & G-U &  & CE   & MLL   & B   & B-U & G  & G-U  &  & CE   & MLL   & B  & B-U & G & G-U   &  & CE   & MLL   & B   & B-U & G  & G-U  \\ \hline
 \multirow{4}{*}{\rotatebox{90}{SNLI}} & F1 & 0.890  \newline (0.02) & 0.891 \newline (0.02) & 0.880 \newline 0.30 & 0.882 (0.01) & 0.481 (0.01)   & 0.481 (0.01) & &  0.873 (0.00) &  0.882 (0.09) & 0.885 (0.04) &  0.886 (0.00)    &  0.886 (0.00)     &   0.886 (0.00)     &     &   0.861 (0.00)  & 0.865 (0.01) & 0.869 (0.03) & 0.868 (0.00)    & 0.868 (0.00) &  0.868 (0.00)     & & 0.836 (0.00) & 0.848 (0.04) & 0.845 (0.01) & 0.837 (0.00) & 0.845 (0.01) & 0.837 (0.00)\\
 & MAE & 0.123 (0.01) & 0.122 (0.02) & 0.136 (0.00) & 0.132 (0.02) & 0.624 (0.00) & 0.624 (0.00) & & 0.146 (0.00) & 0.131 (0.11)      & 0.129 (0.00)  & 0.128 (0.00)   & 0.128 (0.00) &  0.128 (0.00)   &        &   0.161 (0.00)    & 0.153 (0.01) &   0.150 (0.00)   &  0.151 (0.00)  & 0.151 (0.00)  & 0.151 (0.00)   &    & 0.191 (0.00) & 0.171 (0.05) & 0.181 (0.00) & 0.189 (0.01) & 0.181 (0.00) & 0.189 (0.01)  \\
 & MSE & 0.152 (0.04) & 0.149 (0.04) & 0.169 (0.01) & 0.160 (0.00) & 0.953 (0.00) & 0.953 (0.00) & & 0.188 (0.00) & 0.156 (0.05)      & 0.159 (0.00) &   0.160 (0.00)   & 0.160 (0.00)  & 0.160 (0.00)   &        &  0.206 (0.00)     & 0.190 (0.00) &  0.190 (0.00)    &  0.191 (0.01)  & 0.191 (0.01)  & 0.191 (0.01)   &    & 0.249 (0.01)  & 0.210 (0.06)  & 0.236 (0.00) & 0.248 (0.02) & 0.236 (0.00) & 0.248 (0.02) \\
 & OK1 & 0.985 (0.01) & 0.9861 (0.01)  & 0.9834 (0.02) & 0.985 (0.00) & 0.835 (0.00) & 0.835 (0.00) & & 0.979 (0.00) & 0.987 (0.02)      &  0.980 (0.00)  & 0.983 (0.00) & 0.983 (0.00) &  0.983 (0.00)    &       &   0.977 (0.00)     &   0.981 (0.02)    & 0.980 (0.00)  & 0.980 (0.01)   & 0.980 (0.01) &   0.980 (0.01)    &        &   0.971 (0.00) & 0.980 (0.00) & 0.972 (0.00) & 0.970 (0.00) & 0.972 (0.00) & 0.970 (0.00)\\
\hline
\multirow{4}{*}{\rotatebox{90}{YELP}} & F1 & 0.635 (0.02) & 0.638 (0.02) & 0.635 (0.03)  & 0.631 (0.03) & 0.601 (0.00) & 0.601 (0.00)  &  &  0.618 (0.02)  &   0.624 (0.02) & 0.620 (0.54)  &  0.615 (0.05) & 0.536 (0.00)     &  0.536 (0.00)     &        &   0.602 (0.02)    & 0.607 (0.02) &  0.602 (0.00) & 0.558 (0.00)      &  0.431 (0.00)   & 0.431 (0.00)   &    & 0.581 (0.02) & 0.585 (0.02) & 0.570 (0.01) & 0.271 (0.07) & 0.376 (0.05) & 0.376 (0.05) \\
 & MAE & 0.413 (0.06) & 0.407 (0.01) & 0.417 (0.05) & 0.424 (0.00) & 0.447 (0.01) & 0.447 (0.01) & &  0.438 (0.02)   &  0.426 (0.02) &   0.437 (0.00) & 0.441 (0.00)   &  0.527 (0.00) &  0.527 (0.00)    &       &   0.463 (0.03)     &   0.453 (0.04)    & 0.466 (0.01)  &   0.531 (0.00)   &   0.644 (0.00)    &   0.644 (0.00)     &   & 0.500 (0.02) & 0.487 (0.05) & 0.511 (0.01) & 0.858 (0.14) & 0.633 (0.07) & 0.633 (0.07) \\
 & MSE & 0.539 (0.03) & 0.518 (0.01) & 0.561 (0.01) & 0.571 (0.01) & 0.595 (0.02) & 0.595 (0.02) & &  0.592 (0.06)    &  0.555 (0.05) & 0.596 (0.02)  & 0.600 (0.00)    &  0.749 (0.00)  &    0.749 (0.00)         &        & 0.643 (0.02)  & 0.602 (0.02)  &  0.663 (0.03) & 0.805 (0.01)      &    0.999 (0.00)    & 0.999 (0.00)    & & 0.731 (0.02) &  0.674 (0.03) & 0.723 (0.02) & 2.214 (0.32) & 0.834 (0.15) & 0.834 (0.15)\\
 & OK1 & 0.963 (0.01) & 0.965 (0.03) & 0.960 (0.01) & 0.959 (0.00) & 0.955 (0.00) & 0.955 (0.00) & & 0.957 (0.00)      &  0.960 (0.08)   & 0.956 (0.00) &   0.957 (0.00)    & 0.928 (0.00) &   0.928 (0.00)          &        & 0.951 (0.00)  & 0.956 (0.01)  &  0.946 (0.00)  & 0.926 (0.00) & 0.883 (0.00)   &  0.883 (0.00) &    &   0.941 (0.00)  & 0.944 (0.00) & 0.939 (0.00) & 0.926 (0.03) & 0.929 (0.02) & 0.929 (0.02)\\
\hline
\multirow{4}{*}{\rotatebox{90}{SST5}} & F1  & 0.484 (0.01) & 0.491 (0.02) & 0.51 (1.75) & 0.421 (0.07) & 0.487 (0.02)  & 0.487 (0.02) &   &    0.442 (0.02)    &   0.468 (0.03)    &  0.446 (2.55)  &  0.354 (0.05)    &  0.476 (0.00) &   0.476 (0.00)   &       &         0.415 (0.03)    & 0.440 (0.04) &  0.423 (2.29)    &  0.267 (0.09) & 0.316 (0.01)    & 0.316 (0.01)  & &  0.417 (0.02)  & 0.428 (0.02) & 0.358 (1.97) & 0.108 (0.02) & 0.274 (0.02) & 0.274 (0.02) \\
 & MAE & 0.576 (0.02) & 0.574 (0.01)  & 0.543 (0.04)  & 0.579 (0.03) & 0.585 (0.01)  & 0.585 (0.01) &  &  0.620 (0.01)    &   0.600 (0.02)     &  0.585 (0.01) & 0.749 (0.10)  & 0.595 (0.00) &  0.595 (0.00)    &       &   0.652 (0.04)     &   0.620 (0.04)    & 0.619 (0.03) &  1.026 (0.27)    &  0.966 (0.03)     &  0.966 (0.03)  &    &  0.697 (0.02) & 0.662 (0.01) & 0.651 (0.01) & 1.259 (0.05) & 1.043 (0.02) & 1.043 (0.02)\\
 & MSE & 0.760 (0.02) & 0.756 (0.02) & 0.683 (0.04)   & 0.755 (0.07) & 0.802 (0.02)   & 0.802 (0.02) &  &   0.845 (0.04)   & 0.760 (0.04)      &  0.794 (0.02) & 1.193 (0.26)  &  0.819 (0.01) &  0.819 (0.01)    &       &    0.910 (0.10)    &   0.827 (0.01)    & 0.870 (0.07) &  1.651 (0.08) & 1.740 (0.10)      &  1.740 (0.10)    &  &   1.04 (0.06) & 0.905 (0.01) & 0.872 (0.03) & 2.530 (0.37) & 1.897 (0.19) & 1.897 (0.19)\\
 & OK1 &   0.925 (0.01)   &    0.931 (0.02)   &  0.932 (0.02)  & 0.921 (0.01) & 0.918 (0.00) & 0.918 (0.00) &   & 0.910 (0.08) &      0.929 (0.01)      &  0.927 (0.01)      & 0.858 (0.02)  & 0.912 (0.00)  &   0.912 (0.00)   &       &    0.902 (0.01)    &    0.918 (0.02)   & 0.911 (0.01) &  0.721 (0.01) & 0.769 (0.01)       &  0.769 (0.01)      &   &  0.875 (0.01) & 0.898 (0.02) & 0.916 (0.01) &  0.618 (0.03) & 0.734 (0.01) & 0.734 (0.01)\\
\hline
\multirow{4}{*}{\rotatebox{90}{ \parbox{0.75cm}{Amazon \newline Reviews} }} & F1  & 0.586 (0.04) & 0.589 (0.04) & 0.585 (0.03)  & 0.536 (0.00) & 0.536 (0.00)    & 0.536 (0.00) &    & 0.573 (0.00)  & 0.579 (0.01) &  0.586 (0.02) & 0.584 (0.00)      & 0.584 (0.00) &  0.584 (0.00)    &       &  0.563 (0.00)      &   0.572 (0.02)  &  0.572 (0.01) &   0.565 (0.01)   &  0.565 (0.01)    &  0.565 (0.01)  &        &  0.534 (0.01)  & 0.553 (0.03)  & 0.546 (0.01) & 0.559 (0.00) & 0.559 (0.00) & 0.559 (0.00) \\
 & MAE & 0.485 (0.06) & 0.476 (0.06)  &  0.483 (0.01) & 0.549 (0.00) & 0.549 (0.00) & 0.549 (0.00) &    & 0.505 (0.00) &  0.497 (0.01) & 0.480 (0.00) & 0.479 (0.00)     &  0.479 (0.00) &  0.479 (0.00)    &       &    0.520 (0.00)    &   0.503 (0.07)    &  0.502 (0.02)  &  0.514 (0.01)    &   0.479 (0.00)    &  0.479 (0.00)   &   &  0.56 (0.01) & 0.528 (0.05) & 0.540 (0.02) & 0.516 (0.00) & 0.516 (0.00) & 0.516 (0.00)\\
 & MSE & 0.675 (0.01) & 0.634 (0.01) & 0.664 (0.02) & 0.786 (0.00) & 0.786 (0.00)  & 0.786 (0.00) &      & 0.707 (0.01) & 0.683 (0.03)    &   0.655 (0.01) & 0.643 (0.00) &  0.643 (0.00) &  0.643 (0.00)    &       &  0.739 (0.02)      &   0.689 (0.02)    & 0.698 (0.05)  & 0.731 (0.04)   &  0.731 (0.04)     &  0.731 (0.04)  &    &   0.835 (0.04) & 0.708 (0.01) & 0.766 (0.06) & 0.689 (0.00) & 0.689 (0.00) & 0.689 (0.00)\\
 & OK1 & 0.938 (0.03) & 0.945 (0.03) & 0.939 (0.01) & 0.923 (0.00) & 0.923 (0.00) & 0.923 (0.00) &      & 0.932 (0.00)  &  0.935 (0.00)    &   0.942 (0.00) &  0.945 (0.00) & 0.945 (0.00)  &   0.945 (0.00)   &       &   0.929 (0.00)     &    0.938 (0.03)   & 0.935 (0.01) & 0.930 (0.00) &   0.930 (0.00)    & 0.930 (0.00)    &   &  0.913 (0.00) & 0.934 (0.02) & 0.927 (0.01) & 0.938 (0.00) & 0.938 (0.00) & 0.938 (0.00)\\
\hline

\end{tabular}
\caption{Summary of all the results}
\label{tab:main_table}
\end{table*}


==> main_table_real.tex <==
\begin{table*}[]
\tiny
\begin{tabular}{cp{0.20cm}p{0.20cm}p{0.20cm}p{0.20cm}p{0.20cm}p{0.20cm}p{0.20cm}|p{0.005cm}|p{0.20cm}p{0.20cm}p{0.20cm}p{0.20cm}p{0.20cm}p{0.20cm}|p{0.05cm}|p{0.20cm}p{0.20cm}p{0.20cm}p{0.20cm}p{0.20cm}p{0.20cm}|p{0.05cm}|p{0.20cm}p{0.20cm}p{0.20cm}p{0.20cm}p{0.20cm}p{0.20cm}}
 &     & \multicolumn{6}{c}{100 \%} &  & \multicolumn{6}{c}{50 \%} &  & \multicolumn{6}{c}{25 \%} &  & \multicolumn{6}{c}{10 \%} \\
  &     & CE   & MLL   & B & B-U & GPT  & G-U &  & CE   & MLL   & B   & B-U & G  & G-U  &  & CE   & MLL   & B  & B-U & G & G-U   &  & CE   & MLL   & B   & B-U & G  & G-U  \\ \hline
 \multirow{4}{*}{\rotatebox{90}{SNLI}} & F1 & 0.890  \newline (0.02) & 0.891 \newline (0.02) & 0.885 (0.30) & 0.882 (0.01) & 0.776 (0.00) &  0.861 (0.00) & &  0.873 (0.00) &  0.882 (0.09) & 0.885 (0.04) &  0.884 (0.00) & 0.654 (0.00) & 0.818 (0.00)   &     &   0.861 (0.00)  & 0.865 (0.01) & 0.869 (0.03) & 0.868 (0.00) & 0.527 (0.01)  & 0.732 (0.00)  & & 0.836 (0.00) & 0.848 (0.04) & 0.845 (0.01) & 0.837 (0.00) & 0.389 (0.01) & 0.430 (0.02)\\
 & MAE & 0.123 (0.01) & 0.122 (0.02) & 0.128 (0.00) & 0.132 (0.02) & 0.261 (0.00) & 0.156 (0.00) & & 0.146 (0.00) & 0.131 (0.11) & 0.129 (0.00)  & 0.130 (0.00) & 0.424 (0.00)  & 0.211 (0.00)  &        &   0.161 (0.00)    & 0.153 (0.01) &   0.150 (0.00)   &  0.151 (0.00)  &  0.599 (0.02) &  0.312 (0.00)  &    & 0.191 (0.00) & 0.171 (0.05) & 0.181 (0.00) & 0.189 (0.01)  & 0.811 (0.01) & 0.711 (0.02)\\
 & MSE & 0.152 (0.04) & 0.149 (0.04) & 0.157 (0.01) & 0.160 (0.00) & 0.338 (0.00) & 0.193 (0.00) & & 0.188 (0.00) & 0.156 (0.05)      & 0.159 (0.00) &   0.161 (0.00) & 0.596 (0.00)  & 0.272 (0.00) &        &  0.206 (0.00)     & 0.190 (0.00) &  0.190 (0.00)    &  0.191 (0.01)  & 0.878 (0.04)  &  0.405 (0.00)  &    & 0.249 (0.01)  & 0.210 (0.06)  & 0.236 (0.00) & 0.248 (0.02) & 1.263 (0.04) & 1.051 (0.04)\\
 & OK1 & 0.985 (0.01) & 0.9861 (0.01)  & 0.985 (0.02) & 0.985 (0.00) & 0.961 (0.00) & 0.981 (0.00) & & 0.979 (0.00) & 0.987 (0.02)      &  0.980 (0.00)  & 0.984 (0.00) & 0.913 (0.00) &  0.969 (0.00)    &       &   0.977 (0.00)     &   0.981 (0.02)    & 0.980 (0.00)  & 0.980 (0.01) & 0.860 (0.01) & 0.953 (0.00)      &        &   0.971 (0.00) & 0.980 (0.00) & 0.972 (0.00) & 0.970 (0.00) & 0.774 (0.01) & 0.830 (0.01)\\
\hline
\multirow{4}{*}{\rotatebox{90}{YELP}} & F1 & 0.635 (0.02) & 0.638 (0.02) & 0.635 (0.03)  & 0.631 (0.03) & 0.601 (0.00) & 0.648 (0.00) &  &  0.618 (0.02)  &   0.624 (0.02) & 0.620 (0.54)  &  0.615 (0.05) & 0.536 (0.00) & 0.610 (0.00)      &        &   0.602 (0.02)    & 0.607 (0.02) &  0.602 (0.00) & 0.558 (0.00)      &  0.431 (0.00)   & 0.511 (0.02) &    & 0.581 (0.02) & 0.585 (0.02) & 0.570 (0.01) & 0.271 (0.07) & 0.376 (0.05) & 0.307 (0.06) \\
 & MAE & 0.413 (0.06) & 0.407 (0.01) & 0.417 (0.05) & 0.424 (0.00) & 0.447 (0.01) & 0.388 (0.00) & &  0.438 (0.02)   &  0.426 (0.02) &   0.437 (0.00) & 0.441 (0.00)   &  0.527 (0.00) &  0.438 (0.00)    &       &   0.463 (0.03)     &   0.453 (0.04)    & 0.466 (0.01)  &   0.531 (0.00)   &   0.644 (0.00)    &  0.547 (0.02) &   & 0.500 (0.02) & 0.487 (0.05) & 0.511 (0.01) & 0.858 (0.14) & 0.633 (0.07) & 0.977 (0.11) \\
 & MSE & 0.539 (0.03) & 0.518 (0.01) & 0.561 (0.01) & 0.571 (0.01) & 0.595 (0.02) & 0.486 (0.00) & &  0.592 (0.06)    &  0.555 (0.05) & 0.596 (0.02)  & 0.600 (0.00)    &  0.749 (0.00)  & 0.570 (0.00)   &        & 0.643 (0.02)  & 0.602 (0.02)  &  0.663 (0.03) & 0.805 (0.01)      &    0.999 (0.00) & 0.746 (0.03)   & & 0.731 (0.02) &  0.674 (0.03) & 0.723 (0.02) & 2.214 (0.32) & 0.834 (0.15) & 1.724 (0.38)\\
 & OK1 & 0.963 (0.01) & 0.965 (0.03) & 0.960 (0.01) & 0.959 (0.00) & 0.955 (0.00) & 0.970 (0.00) & & 0.957 (0.00)      &  0.960 (0.08)   & 0.956 (0.00) &   0.957 (0.00)    & 0.928 (0.00) & 0.957 (0.00)  &        & 0.951 (0.00)  & 0.956 (0.01)  &  0.946 (0.00)  & 0.926 (0.00) & 0.883 (0.00) & 0.917 (0.00) &    &   0.941 (0.00)  & 0.944 (0.00) & 0.939 (0.00) & 0.926 (0.03) & 0.929 (0.02) & 0.727 (0.07) \\
\hline
\multirow{4}{*}{\rotatebox{90}{SST5}} & F1  & 0.484 (0.01) & 0.491 (0.02) & 0.508 (0.01) & 0.463 (0.07) & 0.487 (0.02)  & 0.150 (0.01) &   &    0.442 (0.02)    &   0.468 (0.03)    &  0.445 (0.02)  &  0.401 (0.05)    &  0.476 (0.00) & 0.094 (0.00) &       &         0.415 (0.03)    & 0.440 (0.04) &  0.423 (0.03)    &  0.347 (0.09) & 0.316 (0.01) & 0.077 (0.01) & &  0.417 (0.02)  & 0.428 (0.02) & 0.358 (0.03) & 0.172 (0.02) & 0.274 (0.02) & 0.067 (0.01)\\
 & MAE & 0.576 (0.02) & 0.574 (0.01)  & 0.543 (0.01)  & 0.557 (0.03) & 0.585 (0.01)  & 1.175 (0.04) &  &  0.620 (0.01)    &   0.600 (0.02)     &  0.585 (0.01) & 0.616 (0.10)  & 0.595 (0.00) & 1.140 (0.00)  &       &   0.652 (0.04)     &   0.620 (0.04)    & 0.619 (0.04) &  0.732 (0.27)    &  0.966 (0.03) & 1.488 (0.30)   &    &  0.697 (0.02) & 0.662 (0.01) & 0.651 (0.10) & 1.381 (0.05) & 1.043 (0.02) & 1.649 (0.36)\\
 & MSE & 0.760 (0.02) & 0.756 (0.02) & 0.683 (0.02)   & 0.722 (0.07) & 0.802 (0.02) & 2.007 (0.10) &  &   0.845 (0.04)   & 0.760 (0.04)      &  0.794 (0.04) & 0.805 (0.02)  &  0.819 (0.01) &  1.843 (0.04)  &       &    0.910 (0.10)    &   0.827 (0.01)    & 0.870 (0.12) &  1.169 (0.08) & 1.740 (0.10) & 3.394 (1.41)   &  &   1.04 (0.06) & 0.905 (0.01) & 0.871 (0.25) & 3.035 (0.37) & 1.897 (0.19) & 4.130 (1.67)\\
 & OK1 &   0.925 (0.01)   &    0.931 (0.02)   &  0.932 (0.01)  & 0.929 (0.01) & 0.918 (0.00) & 0.666 (0.01) &   & 0.910 (0.08) &      0.929 (0.01)      &  0.927 (0.01) & 0.912 (0.02)  & 0.912 (0.00)  & 0.687 (0.00) &       &    0.902 (0.01)    &    0.918 (0.02)   & 0.911 (0.02) &  0.855 (0.01) & 0.769 (0.01) & 0.568 (0.10)        &   &  0.875 (0.01) & 0.898 (0.02) & 0.915 (0.05) &  0.595 (0.03) & 0.734 (0.01) & 0.513 (0.12) \\
\hline
\multirow{4}{*}{\rotatebox{90}{ \parbox{0.75cm}{Amazon \newline Reviews} }} & F1  & 0.586 (0.04) & 0.589 (0.04) & 0.585 (0.03)  & 0.590 (0.02) & 0.522 (0.00) & 0.574 (0.00)  &    & 0.573 (0.00)  & 0.579 (0.01) &  0.586 (0.02) & 0.584 (0.00) & 0.449 (0.01)  &  0.517 (0.01)    &       &  0.563 (0.00)      &   0.572 (0.02)  &  0.572 (0.01) &   0.565 (0.01) & 0.402 (0.00) & 0.411 (0.01) &        &  0.534 (0.01)  & 0.553 (0.03)  & 0.544 (0.01) & 0.556 (0.00) & 0.389 (0.00) & 0.200 (0.04)\\
 & MAE & 0.485 (0.06) & 0.476 (0.06)  &  0.483 (0.01) & 0.466 (0.01) & 0.573 (0.01) & 0.494 (0.00) &    & 0.505 (0.00) &  0.497 (0.01) & 0.480 (0.00) & 0.479 (0.00) & 0.678 (0.00) & 0.567 (0.01) &       &    0.520 (0.00)    &   0.503 (0.07)    &  0.502 (0.02)  &  0.514 (0.01) & 0.773 (0.00)& 1.196 (0.09) &   &  0.56 (0.01) & 0.528 (0.05) & 0.541 (0.02) & 0.519 (0.00) & 0.813 (0.00) & 1.196 (0.09)\\
 & MSE & 0.675 (0.01) & 0.634 (0.01) & 0.664 (0.02) & 0.624 (0.00)& 0.848 (0.04)  & 0.677 (0.01) &      & 0.707 (0.01) & 0.683 (0.03)    &   0.655 (0.01) & 0.643 (0.00) & 1.085 (0.01) & 0.801 (0.02)  &       &  0.739 (0.02)      &   0.689 (0.02)    & 0.698 (0.05)  & 0.731 (0.04) &  1.348 (0.01) & 2.319 (0.29) &    &   0.835 (0.04) & 0.708 (0.01) & 0.767 (0.06) & 0.695 (0.00) & 1.475 (0.01) & 2.319 (0.29)\\
 & OK1 & 0.938 (0.03) & 0.945 (0.03) & 0.939 (0.01) & 0.945 (0.00) & 0.911 (0.00) & 0.938 (0.00)  &      & 0.932 (0.00)  &  0.935 (0.00)    &   0.942 (0.00) &  0.945 (0.00) & 0.864 (0.00) & 0.912 (0.00)  &       &   0.929 (0.00)     &    0.938 (0.03)   & 0.935 (0.01) & 0.930 (0.00) &  0.825 (0.00) & 0.638 (0.04) &   &  0.913 (0.00) & 0.934 (0.02) & 0.925 (0.01) & 0.937 (0.00) & 0.807 (0.00) & 0.638 (0.04) \\
\hline

\end{tabular}
\caption{Summary of all the results}
\label{tab:main_table_real}
\end{table*}


==> mse_plots_uninformed_vs_informed.tex <==


\begin{figure}[!h]
\centering
\begin{minipage}{.24\textwidth}
  \centering
  \includegraphics[width=\linewidth]{SNLI_MSE.pdf}
  \label{fig:test11}
\end{minipage}%

\begin{minipage}{.24\textwidth}
  \centering
  \includegraphics[width=\linewidth]{SST5_MSE.pdf}
  \label{fig:test21}
\end{minipage}%
\begin{minipage}{.24\textwidth}
  \centering
  \includegraphics[width=\linewidth]{amazon_review_MSE.pdf}
  \label{fig:test22}
\end{minipage}%
\caption{\small Effect of informative vs non-informative prompts on ordinal metric (MSE).}
\label{fig:mse_random}
\end{figure}


==> off1_plots_uninformed_vs_informed.tex <==


\begin{figure}[!h]
\centering
\begin{minipage}{.24\textwidth}
  \centering
  \includegraphics[width=\linewidth]{SNLI_OFF1.pdf}
  \label{fig:test11}
\end{minipage}%

\begin{minipage}{.24\textwidth}
  \centering
  \includegraphics[width=\linewidth]{SST5_OFF1.pdf}
  \label{fig:test21}
\end{minipage}%
\begin{minipage}{.24\textwidth}
  \centering
  \includegraphics[width=\linewidth]{amazon_review_OFF1.pdf}
  \label{fig:test22}
\end{minipage}%
\caption{\small Effect of informative vs non-informative prompts on ordinal metric (OB1).}
\label{fig:random_prompt}
\end{figure}


==> plots_uninformed_vs_informed.tex <==







\begin{figure*}
\begin{minipage}{.25\textwidth}
    \begin{figure}[H]
    \includegraphics[width=1.2\textwidth]{radial_plot_karan_wo_yelp_llama.pdf}
    \caption{\small \% samples following UM property.}
    \label{fig:unimodal}
\end{figure}
\end{minipage}
\hspace{0.04\linewidth}
\begin{minipage}{.7\textwidth}
    \begin{figure}[H]
\centering
\begin{minipage}{.3\textwidth}
  \centering
  \includegraphics[width=1.2\linewidth]{SNLI_F1.pdf}
  \label{fig:test11}
\end{minipage}%
\begin{minipage}{.3\textwidth}
  \centering
  \includegraphics[width=1.2\linewidth]{SST5_F1.pdf}
  \label{fig:test21}
\end{minipage}%
\begin{minipage}{.3\textwidth}
  \centering
  \includegraphics[width=1.2\linewidth]{Amazon_Reviews_F1.pdf}
  \label{fig:test22}
\end{minipage}%
\caption{\small Effect of informative vs non-informative prompts on classification (F1-score).}
\label{fig:random_prompt}



\end{figure}
\end{minipage}
    
\end{figure*}

